Discovering Hierarchical Processes Using Flexible Activity Trees for Event Abstraction

Processes, such as patient pathways, can be very complex, comprising of hundreds of activities and dozens of interleaved subprocesses. While existing process discovery algorithms have proven to construct models of high quality on clean logs of structured processes, it still remains a challenge when the algorithms are being applied to logs of complex processes. The creation of a multi-level, hierarchical representation of a process can help to manage this complexity. However, current approaches that pursue this idea suffer from a variety of weaknesses. In particular, they do not deal well with interleaving subprocesses. In this paper, we propose FlexHMiner, a three-step approach to discover processes with multi-level interleaved subprocesses. We implemented FlexHMiner in the open source Process Mining toolkit ProM. We used seven real-life logs to compare the qualities of hierarchical models discovered using domain knowledge, random clustering, and flat approaches. Our results indicate that the hierarchical process models that the FlexHMiner generates compare favorably to approaches that do not exploit hierarchy.

==> files/040researchproblem.tex <==
\subsection{Research Problem - Grouping Patients}


Traditional trace clustering aims to divide the traces of a log into clusters, such that the traces of the same cluster show more homogenous behavior than the traces of different clusters. 
In the healthcare domain, we are facing a very large, complex data set and abundant domain knowledge. As discussed at the end of~\autoref{sec:relatedwork}, 
%, as depicted in~\autoref{fig:Untitled2}. 
%
%\begin{itemize}
%\item
%Firstly, we . %\mi{PI}evertheless, the right number of clusters is still unknown. 
%
%\item
%\draft{It has been difficult to evaluate or to validate the quality of such a large clustering, as the resulting clusters were often not inline with those of medical experts. 
%\item 
%Moreover, the quality of each cluster is highly context-dependent; discussing with a different expert, the patients may be grouped based on different criteria or features~\cite{DBLP:journals/ijmi/BeekGK05}.
%
%For instance, the Dutch patient classification system (DBC) consists of more than two thousands distinct diagnostic codes optimized for grouping patient pathway from a financial perspective~\cite{schreyogg2006methods}. Multiple codes are used for referring to the same disease or the other way around. Experts therefore use additional attributes to define their patient groups of interest~\cite{DBLP:journals/ijmi/BeekGK05}. }
%\end{itemize}
%
we would like to (1) handle such a large data set, to (2) incorporate, leverage, and put more emphasis on the domain knowledge, in order to obtain clusters that are more in line with those of medical experts, while requiring little effort from such experts, and to (3) be able to find the clusters accurately and validate clusters quality, we propose the following. 

We assume that medical experts can provide a small sample set $P$ of the patients that belong to a patient group $\hat{C}$ of interest. %for example a set of patient ids \subset \hat{C}$. 
This requires little effort from their side. 
%(1)
%\todo{sum the problems and therefore the solution}
%\textcolor[rgb]{1,0,0}{In such cases where domain knowledge is of important and has specific meanings, we may ask the domain expert to give a sample set. }
%
%Let us assume that there is such a sample set $P$ of the patients given that should be clustered into one group $G$ (i.e., $P \subset G \subset \mi{PI}$). 
%Note that the group $\hat{C}$ is unknown; 
%\draft{
In principle, medical experts, doctors in particular, would be able to exhaustively define the group, but this would require too much effort when $\hat{C}$ gets large and would be difficult to repeat for other groups. Therefore, we assume that $\hat{C}$ is unknown. 
We use the available event data of all patients including $P$, aiming to find a cluster $C$ in such a way that $C$ is as close to the group $\hat{C}$ as possible (i.e., the highest recall and precision possible).
We do this separately for each group $\hat{C}_i$ where the sample set $P_i$ is available. 
%
%Let us assume that we have the patient ids $\mi{PI} = \{n_1, \cdots, n_{|\mi{PI}|}\}$, and the event log $L$ of the patients $\mi{PI}$,the set of activities $A$, and the diagnostic codes $D$ as our starting point. Now, a subset $P \subset \mi{PI}$ of the patients that belongs to the group $G$ are provided to us by the domain expert (e.g., the doctor). But the group $G$ is unknown. We would like to compute a set $\leftcenterhat{G} \subset \mi{PI}$ of patients using $P$, such that the set difference between $G$ and $\leftcenterhat{G}$ is minimized. 
%
To generalize, we define the partial trace clustering formally as follows. 

\begin{definition}[Partial Trace Clustering]
%Let $A$ be a set of activities, 
Let $L = \{\sigma_1, \cdots, \sigma_n\}$ be the event log, and $\mi{PI} = \{\pi_{pi}(\sigma_1), \cdots, \pi_{pi}(\sigma_n)\}$ the set of cases of $L$. Let $P_1, P_2, \cdots, P_x \subset \mi{PI}$ be the sets of samples that respectively belong to clusters $\hat{C}_1, \hat{C}_2, \cdots, \hat{C}_x$, provided by experts (e.g., a doctor), with $x \in \mathbb{N}$. We would like to find the clusters $C_1, C_2, \cdots, C_x \subset \mi{PI}$, such that the set difference between $C_i$ and $\hat{C}_i$ is minimized. 
\end{definition}

Note that clusters $C_1, C_2, \cdots, C_x$ can be non-overlapping or form an incomplete clustering of $\mi{PI}$ (i.e., $ C_1 \cup \cdots \cup C_x \subseteq \mi{PI}$). These properties of a partial trace clustering can be exploited. We do not have to find all clusters or to compute a complete clustering. It allows us to mine, cluster, and validate each cluster independently. 
%\draft{Moreover, it only requires little input from the experts. Instead of coming up with the specific definition or criteria of the group, which would require many manual work and discussions~\cite{}, the experts only have to give a few patients as examples of the group. }


%2. 


%\draft{In general, data of patients related to their clinical pathways is made available, including the diagnostic codes and the activities executed. We aim to cluster patients into meaningful groups by using (1) the original patient diagnostic classification (known in the Netherlands as Diagnostic and Billing Code (DBC)), (2) the activities recorded for each patients, and only (3) a small sample of patients provided by the medical expert.}

%If we consider each patient as a case, then the events can be grouped by patients, and six traces are shown. 
%In general, we would like to cluster the patients into m meaningful groups of diseases. However, such problem is extremely complex due to different reasons. 
%	- First, the data set is too large to do this efficiently. 
%	- Secondly, the clustering is rather domain dependent, highly fluctuate in the opinion of doctors. 
%	- Thirdly, returning thousands of clusters, it would be difficult to validate the quality of clusters as we apply our approach on real data sets. 
%\todo{XL: do we want to mention that existing approaches cluster patients into $k$ clusters. However, formulating the problem in such a way has several disadvantages. Therefore, we did this differently?}


%More specifically, for example, in our data set, the hospital is handling more than 120 thousands of patients and executing more than 4 millions of events per year. In 2017, more than 1.8 thousands of unique DBC and 5 thousand distinct activities have been recorded. The feature space ($\sim 6.8$ thousands) and the number of cases ($\sim 120$ thousands) are too immense. 

%Furthermore, it would be difficult to validate the quality of the hundreds or thousands of clusters we found with the doctors if we apply our approach on real data sets. 

%In this paper, we formulate the research problem as follows. Assuming a sample $P$ of the patients $N$ that should be clustered into one group $G$ is given, we would like to find all other patients in $N \backslash P$ that belong to this group $G$ with the highest recall and precision possible. In this way, we can also validate our results of each cluster independently with the experts and leverage the labeled patients. Additionally, we want the criteria for the grouping to be understandable for medical specialists.

%We have $N = \{n_1, n_2, \cdots, n_m\}$ patients. 

%Formally, given the healthcare activities $A$, the diagnostic codes $D$, the patient ids $N$, the event log $L$ of the patients $N$, and the set of patients $P \subset N$ that belongs to group $G$ labeled by the domain expert (the doctor), we would like to compute a set $\leftcenterhat{G} \subset N$ of patients, such that the set difference between $G$ and $\leftcenterhat{G}$ is minimized. 




==> files/app.tex <==
\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth]{figs/resFitn.pdf}}
\caption{...}
\label{fig:resfit}
\end{figure*}
\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth]{figs/resPrec.pdf}}
\caption{...}
\label{fig:resPrec}
\end{figure*}
\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth]{figs/resGen.pdf}}
\caption{...}
\label{fig:resGen}
\end{figure*}
\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth]{figs/resCFC.pdf}}
\caption{...}
\label{fig:resGen}
\end{figure*}

\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth]{figs/resHAIMvsNonHier3.pdf}}
\caption{The first five plots show fitness (on x-axis) and precision (on y-axis) scores of subprocesses discovered by the \aam (in red) versus the flat-model discovered by IMf (in blue), using the BPIC15 logs; the second five charts show the generalization and CFC complexity scores.(TODO: this figure is not up-to-date, but the new figure shows similar results)}
\label{fig:resHAIMvsNonHier}
\end{figure*}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.49\textwidth]{figs/resHAIMvsNonHier1217.pdf}}
\caption{The fitness, precision, generalization, and CFC complexity scores of subprocesses discovered by the \aam (in red) versus the flat-model discovered by IMf (in blue), using the BPIC12 and BPIC17f logs (TODO: this figure is not up-to-date, but the new figure shows similar results).}
\label{fig:resHAIMvsNonHier1217}
\end{figure}

%


\begin{figure*}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[height=8cm]{figs/rw_SC_bpic2012spA}  
  \caption{Subprocess Application (A) by SCM.}
  \label{fig:rwSCMvsAAMbpi2012spAscm}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[height=8cm]{figs/rw_aam_BPIC2012spA}  
  \caption{Subprocess Application (A) by \aam}
  \label{fig:rwSCMvsAAMbpi2012spAaam}
\end{subfigure}
\caption{The sub-model (a) discovered by SCM~\cite{DBLP:conf/wcre/LeemansAB18} (on the left) shows a choice behavior between activities, whereas the model (b) by \aam (on the right) shows clearly that \actlabel{A\_SUBMITTED} is mandatory, for the BPIC2012 log.}
\label{fig:rwSCMvsAAMbpi2012spA}
\end{figure*}
